A Longitudinal Analysis of Bloated Java Dependencies

We study the evolution and impact of bloated dependencies in a single software ecosystem: Java/Maven. Bloated dependencies are third-party libraries that are packaged in the application binary but are not needed to run the application. We analyze the history of 435 Java projects. This historical data includes 48,469 distinct dependencies, which we study across a total of 31,515 versions of Maven dependency trees. Bloated dependencies steadily increase over time, and 89.02% of the direct dependencies that are bloated remain bloated in all subsequent versions of the studied projects. This empirical evidence suggests that developers can safely remove a bloated dependency. We further report novel insights regarding the unnecessary maintenance efforts induced by bloat. We find that 22% of dependency updates performed by developers are made on bloated dependencies and that Dependabot suggests a similar ratio of updates on bloated dependencies.

==> old-text.tex <==
%old abstract


% context Software applications are bloated. They include a significant portion of code that is not necessary to run the application correctly. 
Motivated by the negative impact of software bloat on security, performance, and maintenance, several works have proposed techniques to remove bloat. 
However, no work has analyzed how bloat evolves over time or how it emerges in software projects. In particular, a concern when removing bloated code is to know if it might be useful in subsequent versions of the application.
In this work, we  study the evolution and emergence of bloat in a single software ecosystem: Java / Maven. Bloated dependencies are third-party libraries that are packaged in the application binary but are not needed to run the application. %These libraries are either directly declared by developers in configuration files or induced transitively through direct dependencies.
% data 
We analyze the history of \nbProjects Java projects. This historical data includes \nbDependencies distinct dependencies, which we study across a total of \nbCommits versions of Maven dependency trees.
% results
We empirically demonstrate the constant increase of the amount of bloated dependencies over time. A key finding of our analysis is that \ProbBloatedDirect of the  direct dependencies that are bloated  remain bloated in all subsequent versions of the studied projects. This empirical evidence suggests that developers can safely remove a bloated dependency. We further report novel insights regarding the unnecessary maintenance efforts induced by bloat, we identify that \np[\%]{22} of dependency updates are made on bloated dependencies.


% abstract
%Bloated dependencies are third-party libraries that are needlessly part of software projects. These libraries are either directly declared by developers in configuration files or induced transitively through direct dependencies. This intriguing concept was introduced in 2019 by Valero and colleagues, who showed that such dependencies are systematically present in the Maven ecosystem. This paper presents a novel analysis of bloated dependencies.
% data
%We look at the history \nbProjects Java projects to perform a longitudinal analysis of the evolution of bloated dependencies in these projects. To do so, we rely on \depclean to analyze the status of \nbDependencies distinct dependencies in \nbCommits commits that touch the \pom file of the projects.
% results
%Our results show that, overall, the number of bloated dependencies tend to grow over time.  Meanwhile, once a dependency becomes bloated, it is very likely that it remains bloated. We report novel insights regarding the waste of maintenance effort associated with updating bloated direct dependencies. This empirical evidence suggests that developers should take immediate actions to appropriately handle bloated dependencies.


% context
The reuse of third-party libraries has become a prevailing practice in modern software development.
Nowadays, package managers facilitate this practice, serving as an interface between the projects and its packaging ecosystem~\cite{Decan2019}.
For example, Maven\footnote{\url{https://maven.apache.org}} facilitates all the tasks associated to the different phases of the software build, from  compilation to its release to the Maven Central repository.\footnote{\url{https://mvnrepository.com}}
When using these artifacts as Maven dependencies, developers only need to add a few lines of code to the \pom file of their projects.
This minimal modification has a tremendous impact on the size and maintainability of the project~\cite{Cox2019}.
Developers now face new challenges associated to the update~\cite{Kula2018}, migration~\cite{Alrubaye2019}, quality assurance~\cite{Salza2020}, management of licences~\cite{Wu2017}, and resolution of dependency conflicts~\cite{Wang2018}.

Soto-Valero~\etal~\cite{Valero2020} recently introduced the concept of \textit{bloated dependencies}.
These are software artifacts that are unnecessarily part of software projects, \ie when the dependency is removed from the project, it still builds successfully.
This is a novel and intriguing concept.
According to their results, the Maven ecosystem is permeated of bloated dependencies, and this type of dependencies are present even on very popular and well maintained Java projects.

Bloated dependencies are problematic for several reasons. 
Although being useless, bloated dependencies could embed vulnerable code that can be exploited by attackers.
Since the project's binary includes more code than necessary, this excess of size could significantly affect its deployment in environments with limited resources.
Managing bloated dependencies is also an unnecessary burden for developers, who need to maintain updating dependencies that the project does not require.
In summary, bloated dependencies are an issue for security, for performance, and maintenance.

% problem
The impact of these results call for more research on this topic, which is the motivation of this paper.
First, we want to determine if the number of bloated dependencies in Java projects tend to grow over time, and which are the factors that make a dependency to become bloated or not.
Second, we want to know if the usage status of dependencies changes over time, and how frequently are bloated dependencies being updated by developers.

% contributions
To investigate the presence of bloated dependencies in Java projects over time, we perform an empirical study based on the analysis of \nbProjects open-source projects.
We rely on \depclean, the state-of-the-art tool to detect bloated dependencies in Maven projects.
In total, we analyze the evolution of \nbDependencies distinct dependencies in \nbCommits release and Dependabot commits.
We articulate our study in two parts.













% This paper answers the following global question: \textit{To what extend is dependency usage stable over time?}\\ 

% \noindent This paper has the following hypothesis:

% \begin{itemize}[leftmargin=24pt]
%     \item[\textbf{H1}.] \textbf{Dependency bloat tends to increase over time.} How much? How often? Why?

%     \item[\textbf{H2}.] \textbf{Bloated dependencies waste resources.} How many times developers change the version of dependencies that are bloated? What is the impact of bots on this?
    
%     \item[\textbf{H3}.] \textbf{The usage status of each individual dependency does not evolve  over time.} Is it a dependency that is bloated today likely to remain bloated in the future?
    
%     \item[\textbf{H4}.] \textbf{Some specific maintenance activities lead to the introduction of bloated dependencies} How often dependency bloat appears because of adding/removing dependencies in the POM, or changing the code?
% \end{itemize}

% \noindent Actionable insights for developers:

% \begin{itemize}[leftmargin=24pt]
%     \item[\textbf{I1}.] \textbf{Bloat is a real problem and it increases over time.} We have strong evidence of the existence of this phenomenon.
    
%     \item[\textbf{I2}.] \textbf{Stop updating dependencies that are bloated.} We raise awareness that practice is a waste of resources.

%     \item[\textbf{I3}.] \textbf{You can trust the diagnosis of debloat tools.} We show that if a dependency is bloated today it is likely that it will be bloated tomorrow.
    
%     \item[\textbf{I4}.] \textbf{Most of the bloat appears because adding/removing dependencies, or refactoring the code.} We recommend developers to be careful when performing this maintainability activity because that might be the time when bloat is introduced in the project.
% \end{itemize}







Software projects usually grow exponentially fast \todo{not sure about the importance of 'fast' here} over time~\cite{Holzmann2015}.

Package managers play an important role in modern software development, providing a pool of reusable artifacts~\cite{Decan2019}.

Previous work has show that most of these artifacts, when used as dependencies, are bloated~\cite{Valero2020}.
This first question aims at determining count trend of bloated dependencies in open-source projects.




% The usage of Java dependencies in Maven is an abstract concept.
% To illustrate the concepts defined previously, we present an example of a typical Maven project $p$.
% In the following, we describe the three principal layers that we consider in this study.




% In this section, we first define the key dependency-related concepts that are the basis of this work.
% Then, we present an illustrative example of these concepts. 

% \todo{I suggest to swap the subsections, the definitions are easier to understand after an example. Also, I think that with definitions of direct dependency and transitive dependency, we don't need to define 'software dependency'}

% \subsection{Definitions}






\[
  f(\mathcal{T}_p) =
  \begin{cases}
    % \text{\emph{inc\_only}} & \text{if $\forall t_i \in \mathcal{T}_p : t_i \geq t_{i-1} \wedge \exists t_j \in \mathcal{T}_p : t_j > t_{j-1}$} \\
    % \text{\emph{dec\_only}} & \text{if $\forall t_i \in \mathcal{T}_p : t_i \leq t_{i-1} \wedge \exists t_j \in \mathcal{T}_p : t_j < t_{j-1}$} \\
    \text{\emph{inc}} & \text{if $slope(lm(\mathcal{T}_p)) > 0 \wedge \exists t_j \in \mathcal{T}_p : t_j < t_{j-1}$} \\
    \text{\emph{dec}} & \text{if $slope(lm(\mathcal{T}_p)) < 0 \wedge \exists t_j \in \mathcal{T}_p : t_j > t_{j-1}$} \\
    \text{\emph{stable}} & \text{if $\forall t_i \in \mathcal{T}_p : t_i = t_{i-1}$} 
    % \text{variable} & \text{otherwise}
  \end{cases}
\]

% A project labelled as \emph{inc\_only} is a project for which the number of bloated dependencies is monotonically increasing.  
% A project labelled as \emph{dec\_only} is a project for which the number of bloated dependencies is monotonically decreasing.
